Towards Optimal and Efficient Best Arm Identification in Linear Bandits

We give a new algorithm for best arm identification in linearly parameterised bandits in the fixed confidence setting. The algorithm generalises the well-known LUCB algorithm of Kalyanakrishnan et al. (2012) by playing an arm which minimises a suitable notion of geometric overlap of the statistical confidence set for the unknown parameter, and is fully adaptive and computationally efficient as compared to several state-of-the methods. We theoretically analyse the sample complexity of the algorithm for problems with two and three arms, showing optimality in many cases. Numerical results indicate favourable performance over other algorithms with which we compare.

==> Algorithm.tex <==
\section{Algorithm}\label{sec:Algorithm}
We now state the main algorithm of this paper formally. Any algorithm for the best arm identification problem has the following algorithmic ingredients: 
\begin{enumerate}
\item a stopping rule: which controls the end of sampling phase and is a function of the past observations and rewards only, 
\item a sampling rule: which determines based on the past play of arms and observations, which arm to pull next; and
\item a recommendation rule: which when the algorithm stops, reports the index of the arm concluded by the algorithm as guess for the best arm.

\end{enumerate}
\textbf{Stopping rule:} The algorithm stops when the ``Advantage" defined in the algorithm becomes non-positive for every arm other than the current best arm $h_*^t.$ 
\begin{align}\label{eq:stopping rule}
\max\limits_{a\in [K]\backslash\{h_*^t \}}Advantage(a) < 0 &\Leftrightarrow \max\limits_{a\in [K]\backslash\{h_*^t \}} \max\limits_{\theta \in \mathcal{E}_t}(\theta^Tx_a-\theta^Tx_{h_*^t}) <0\\
& \Leftrightarrow \max\limits_{a\in [K]\backslash\{h_*^t \}} \theta_t^T(x_a-x_{h_*^t})  + \beta_t\norm{x_a-x_{h_*^t}}_{V_t^{-1}}<0.
\end{align}
\vspace{-0.25cm}

\textbf{Sampling rule:} Play the arm which minimizes the current max Advantage:
\begin{align*}
c_{t+1} \in \argmin\limits_{a\in [K]} \theta_t^T(x_{l_*^t}-x_{h_*^t})  + \beta_t\norm{x_{l_*^t}-x_{h_*^t}}_{{V_t+x_ax_a^T}^{-1}} &= \argmin\limits_{a\in [K]} \norm{x_{l_*^t}-x_{h_*^t}}_{{V_t+x_ax_a^T}^{-1}}.
\end{align*}
By Sherman-Morrison formula, we get $ c_{t+1} = \argmax\limits_{a \in[K]} \abs{\frac{x_a^TV_t^{-1}(x_{h_*^t}-x_{l_*^t})}{\sqrt{1+x_a^TV_t^{-1}x_a}}}. $ In case of a tie, the agent selects an arm uniformly randomly from $c_{t+1}$.\\
\textbf{Recommendation rule:} Once the algorithm stops, the current best arm $h_*^t$ is recommended as the guess for the best arm.

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\begin{algorithm}[H]
 	\caption{{\bf Generalized LUCB}} \label{alg:Main}
 	\begin{algorithmic}[1]
	\State {\bf Input:} $\delta, R, S. $
    \State {\bf Initialize:} $V_0\leftarrow\lambda I$, ${\theta}_0\leftarrow\underline{0}, \beta_0 \leftarrow 1, b_0\leftarrow 0, t\leftarrow 0, STOP \leftarrow 0.$
 	\While {STOP != 0}
 	\State $\mathcal{C}_t \leftarrow \{\theta \in \mathbb{R}^d: \norm{\theta -\theta_t}_{V_t} \leq \beta_t \}$ \Comment{Form the high confidence ellipsoid}
 \State $ 	h_*^t\leftarrow\argmax\limits_{a\in [K]}\theta_t^Tx_a. $\Comment{Current best arm}
 \State $\forall a \in [K]\backslash\{h_*^t \}, Advantage(a) \leftarrow \max\limits_{\theta \in \mathcal{E}_t}(\theta^Tx_a-\theta^Tx_{h_*^t})$
  \If {$\max\limits_{a\in [K]}Advantage(a) < 0$} STOP $\leftarrow$ 1.\Comment{Stopping criterion}
 \Else  
 \State $l_*^t \leftarrow \argmax\limits_{a\in [K]}{Advantage(a)}$\Comment{``Closest" arm}
 \State $c_{t+1} \leftarrow \argmax\limits_{a \in [K]} \abs{\frac{x_a^TV_t^{-1}(x_{h_*^t}-x_{l_*^t})}{\sqrt{1+x_a^TV_t^{-1}x_a}}}.$
 \State Play $a_{t+1} \sim Unif\{ c_{t+1}\}.$
% \State $y_t \sim \mathcal{N}({\theta^*}^Tx_{a_{t}^*},R).$
 \State Receive $y_t$.
 \State $V_{t+1} \leftarrow V_t+ x_{a_{t+1}}{x_{a_{t+1}}}^T.$
 \State $b_{t+1}\leftarrow b_t + y_tx_{a_{t+1}}.$
 \State $\theta_{t+1} \leftarrow V_{t+1}^{-1}b_{t+1}.$
 \State $\beta_{t+1} \leftarrow R\sqrt{2\log \frac{\det(V_{t+1})^{\frac{1}{2}}\det (\lambda I)^{-\frac{1}{2}}}{\delta}}+ \lambda^{\frac{1}{2}}S.$
 \State $t\leftarrow t+1.$
\EndIf
 \EndWhile
 \State \Return $h_*^t.$\Comment{Output the current best arm}
 
 	\end{algorithmic} 
 
 
 \end{algorithm}
 In the next section we provide the proof of correctness of GLUCB and analyze its sample complexity in specific cases.
   
   
   
   
   

==> Generalization.tex <==
\section{Generalization of LUCB using the concept of MaxOverlap}\label{Generalization}
In this section, we introduce a concept that we term "MaxOverlap." This will later motivate the development of our best arm identification algorithm.

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
\subsection{Desideratum}\label{subsec:Connection with a wishful algorithm}
 We wish to design an algorithm which minimizes the overlap of the current confidence ellipsoid with every cone which currently seem to be suboptimal, i.e., all the cones other than the current home cone of $\theta_t$.  
 \begin{definition}[MaxOverlap]
   the MaxOverlap of set $A$ on set $B$ is defined  to be the maximum  distance of set $A$ from the boundary of another set $B$. 
   \begin{align*}
   MaxOverlap(A;B) :=
   \begin{cases}
   \max\limits_{e_A\in A\cap \bar{B}} \min\limits_{e_B \in \partial(\bar{B})\cap A} \norm{e_A-e_B}_2, & if \quad A\cap \bar{B} \neq \emptyset,\\
   0, & \text{otherwise.}
   \end{cases}
   \end{align*}
  Here $\bar{B}$ denotes the closure of the set $B$.
   \end{definition}
%  A schematic diagram of $MaxOverlap$ is shown in figure \ref{fig:MaxOverlap}. \begin{wrapfigure}{r}{0.25\textwidth}
%%  \centering
%  \includegraphics[scale=0.2]{MaxOverlap.png}
%  \caption{A schematic description of the $ MaxOverlap(A;B) $ concept.}
%  \label{fig:MaxOverlap}
%  \end{wrapfigure} 
   Hence, at time $t+1$ play  
   \begin{align*}
   a_{t+1}&:= \argmin\limits_{a=1}^K MaxOverlap\Bigg(\mathcal{E}(\theta_t, V_t+x_ax_a^T); R_{h_t}^c\Bigg)\\
   &= \argmin\limits_{a=1}^K \max\limits_{\substack{\theta\in\mathcal{E} (\theta_t,V_t+ x_ax_a^T),\\ \theta\in R^c_{h_t}}}  \min\limits_{\tilde{\theta}\in \partial(R_{h_t}^c)} \norm{\theta-\tilde{\theta}}_2\\
   &= \argmin\limits_{a=1}^K \max\limits_{\substack{\theta\in\mathcal{E} (\theta_t,V_t+ x_ax_a^T),\\ \theta\in \bigcup\limits_{i \neq h_t} \{\theta':{\theta'}^Tx_i>{\theta'}^Tx_{h_t}\} }}  \min\limits_{\tilde{\theta}\in \bigcup\limits_{i \neq h_t} \{\theta':{\theta'}^Tx_i={\theta'}^Tx_{h_t}\}} \norm{\theta-\tilde{\theta}}_2\\
   &= \argmin\limits_{a=1}^K \max_{i\neq h_t}\max\limits_{\substack{\theta\in\mathcal{E} (\theta_t,V_t+ x_ax_a^T),\\ \theta^Tx_i>\theta^Tx_{h_t}}}  \min\limits_{\tilde{\theta}: \tilde{\theta}^Tx_i=\tilde{\theta}^Tx_{h_t}} \norm{\theta-\tilde{\theta}}_2
   \end{align*}
   
%A wishful choice of the arm to play in order to make the algorithm stop as quickly as possible is as follows. At time $t$ play:
%\[a_{t+1}^{wishful} = \argmin\limits_{a=1}^{K} \max\limits_{\theta \in \mathcal{E}(\theta_t, V_t+x_ax_a^T)}\min\limits_{\tilde{\theta}\in R^c_{h_t}} \norm{\theta-\tilde{\theta}}_2^2. \] 
We have used the fact that $R_{h_t}^c=\sqcup_{i \neq h_t}R_i\equiv \bigcup\limits_{i\neq h_t}\Bigg\{ \tilde{\theta}\in \mathbb{R}^d: \tilde{\theta}^Tx_i>\tilde{\theta}^Tx_{h_t} \Bigg\}.$
The aim of the above choice of arm is to play an arm which will minimize the overlap of the confidence ellipsoid (\textit{of the next round}) with every cone other than the current home cone of $\theta_t$.  
To get a closed form solution for the above, we solve the optimization problem : \[\max\limits_{i\neq h_t} \min\limits_{\tilde{\theta}:\tilde{\theta}^Tx_i > \tilde{\theta}^Tx_{h_t}}\norm{\theta-\tilde{\theta}}_2^2. \]
The problem above can be solved explicitly to obtain:
   \[a_{t+1}= \argmin\limits_{a=1}^{K} \max\limits_{i\neq h_t} \max\limits_{\theta \in \mathcal{E}(\theta_t, V_t+x_ax_a^T)} ({\theta^T(x_i-x_{h_t})})^+ \] 
The agent must stop choosing arms if this value is zero.   
Due to the $max$ over $K-1$ arms the above strategy is inefficient to implement. A slight modification of the above which is easier to implement, is as follows. 
recalling the definition of $HalfSpace$ from Section \ref{Problem}, define the cone ($R(l_t)$) which has the maximum overlap with the \textit{current} cone.
\begin{align*}
l_t &:=\argmax\limits_{i\neq h_t, i\in [K]} MaxOverlap\Bigg(\mathcal{E}(\theta_t, V_t); HalfSpace(i,h_t) \Bigg) \\
&\equiv \argmax_{i\neq h_t}\max\limits_{\substack{\theta\in\mathcal{E} (\theta_t,V_t),\\ \theta^Tx_i>\theta^Tx_{h_t}}}  \min\limits_{\tilde{\theta}: \tilde{\theta}^Tx_i=\tilde{\theta}^Tx_{h_t}} \norm{\theta-\tilde{\theta}}_2\\
&\equiv \argmax\limits_{i\neq h_t} \max\limits_{\theta \in \mathcal{E}(\theta_t, V_t)}\theta^T(x_i-x_{h_t})\\
&=\argmax\limits_{i\neq h_t}\Bigg(\theta_t^T(x_i-x_{h_t}) + \beta_t\norm{x_i-x_{h_t}}_{V_t^{-1}} \Bigg),
\end{align*}
which is straightforward to implement on a computer.
Here $HalfSpace$ is a set defined as $HalfSpace(i;j):=\{\theta:\theta^T(x_i-x_j)>0 \}.$
Then play an arm according to the following rule.\\\\
If $\max\limits_{\theta \in \mathcal{E}(\theta_t, V_t)}\theta^T(x_{l_t}-x_{h_t}) > 0,$ play:
\allowdisplaybreaks
\begin{align*}
a_{t+1} :=& \argmin\limits_{a \in [K]} MaxOverlap\Bigg(\mathcal{E}(\theta_t, V_t+x_ax_a^T); HalfSpace(l_t,h_t) \Bigg) \\
\equiv&\argmin\limits_{a=1}^{K} \max\limits_{\substack{\theta \in \mathcal{E}(\theta_t, V_t+x_ax_a^T)\\\theta^Tx_{l_t}>\theta^Tx_{h_t}}} \min\limits_{\substack{\tilde{\theta}\in \mathbb{R}^d:\\ \tilde{\theta}^Tx_{l_t}=\tilde{\theta}^Tx_{h_t}}} \norm{\theta-\tilde{\theta}}_2\\
=& \argmin\limits_{a=1}^{K} \max\limits_{\theta \in \mathcal{E}(\theta_t, V_t+x_ax_a^T)} \theta^T(x_{l_t}-x_{h_t})\\
=& \argmin\limits_{a=1}^{K}  \Bigg[ \theta_t^T(x_{l_t}-x_{h_t}) +\beta_t\norm{x_{l_t}-x_{h_t}}_{(V_t+x_ax_a^T)^{-1}}\Bigg] \\
=& \argmin\limits_{a=1}^{K}  \norm{x_{l_t}-x_{h_t}}_{(V_t+x_ax_a^T)^{-1}} \\
\equiv& \argmax\limits_{a=1}^K \frac{\abs{x_a^TV_t^{-1}(x_{l_t}-x_{h_t})}}{\sqrt{1+ \norm{x_a}^2_{V_t^{-1}}}}.
\end{align*}
 The equivalence in the last step comes from Sherman-Morrison identity for matrix inverses \cite{Horn:2012:MA:2422911}.
 
 % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
 \subsection{Generalizing LUCB}
  The algorithm we will propose in Section \ref{sec:Algorithm} is a generalization of the celebrated \textit{LUCB} algorithm \cite{Kalyanakrishnan2012PACSS} which is optimal for general unstructured best arm identification problem. In particular, if we consider the case when $d=K$, and the arms being the standard basis $\equiv \{e_1,e_2,\ldots,e_K \}$, we see that the arm $a_2$ in algorithm 1 corresponds to $l_*^t$ which is what LUCB would suggest. Indeed, when $j\neq l_*^t,h_*^t$, $\frac{\abs{x_a^TV_t^{-1}(x_{l_*^t}-x_{h_*^t})}}{\sqrt{1+x_a^TV_t^{-1}x_a}}=0$. However, with $j = l_*^t$ we obtain, $\frac{\abs{x_a^TV_t^{-1}(x_{l_*^t}-x_{h_*^t})}}{\sqrt{1+x_a^TV_t^{-1}x_a}}>0$. Also, it is easy to check the stopping criteria is also similar to LUCB. Hence, algorithm \ref{alg:Main} when applied to the unstructured case, plays the current best and the closest arm simultaneously every time till the algorithm stops.

==> LowerBound.tex <==
\section{Lower Bounds on Sample Complexity}\label{Generallowerbound}
  We begin by restating the result of [\cite{KaufmanOpt}] in the special case of linear bandits. Let $\{x_1,x_2,\ldots,x_K\}$ be a given set of arms  in $\mathbb{R}^d$. Let $\theta$ be any vector in $\mathbb{R}^d$.  For any arbitrary vector $v\in \mathbb{R}^d$, we define $a^*(v):=\argmax\limits_{x_a\in \mathcal{X}}v^Tx_a$. Define the set $Alt(\theta) := \{\xi \in \mathbb{R}^d: a^*(\xi)\neq a^*(\theta) \}$. 
  \begin{lemma}\label{Kaufmann}[Kaufmann etal \cite{KaufmanOpt}]
  Let $\delta \in (0,1).$ For any $\delta-PAC$ strategy and any linear bandit with the unknown parameter vector $\theta \in \mathbb{R}^d$. Let the noise be normal with a variance parameter of $1/2$. Then the expected sample complexity of any strategy
  \beqn
  \mathbb{E}_{\theta}[\tau_{\delta}] \geq T^*(\theta) kl(\delta,1-\delta)
  \eeqn
  where, $kl(x,y) = x\log\frac{x}{y}+ (1-x)\log\frac{1-x}{1-y}$ for $x,y\in [0,1]$ and
  \[T^*(\theta)^{-1} := \sup\limits_{\underline{w}\in \mathcal{P}_K}\inf\limits_{\xi\in Alt(\theta)}\sum\limits_{a=1}^{K}w_aKL(\mathcal{N}(\theta^Tx_a,1/2),\mathcal{N}(\xi^Tx_a,1/2)),\]
 where $\mathcal{P}_K$ is defined as the set of all probability distributions on $\mathcal{X}$ and $KL(P,Q)$ is the KL-divergence between any two probability distributions $P$ and $Q$, and $\mathcal{N}\left(\mu,\sigma^2\right)$ is normal distribution with mean $\mu$ and variance $\sigma^2$.
  \end{lemma}
\subsection{Generalization to The Linear Bandit Problem}
\begin{theorem}[Lower Bound]
Let $\delta \in (0,0.15).$ For any $\delta-PAC$ strategy and any linear bandit problem with the unknown parameter vector $\theta \in \mathbb{R}^d$, the expected sample complexity
\beqn
\frac{\mathbb{E}_{\theta}\left[\tau_{\delta} \right]} {\log\frac{1}{2.4\delta}} \geq \min\limits_{\underline{w}\in \mathcal{P}_K}\max\limits_{a\neq a^*}\frac{\norm{x_a-x_{a^*}}^2_{W^{-1}}}{\Delta_{a}^2}=:H_G.
\eeqn
where the expectation is under $\theta$ and $W:=\sum\limits_{a=1}^{K}w_ax_ax_a^T$, where $\{x_1,x_2,\ldots,x_K\}$ are the arms in $\mathbb{R}^d$ and $a^*:=\argmax\limits_{a\in [K]}\theta^Tx_a.$
\end{theorem}
\begin{proof}(\textit{Sketch})
We obtain a solvable optimization problem by the method of Lagrangian and proceed. The detailed proof is included in Appendix \ref{proof of lower bound}.
\end{proof}
\begin{remark}
For any algorithm whose goal is to identify the best arm, $H_G^{\theta}$ captures the \textit{complexity} of a given problem instance. This term is identical to the complexity term $H_{LB}$ introduced in \cite{soare}. $H_{LB}$ derived in \cite{soare} results from a very different perspective about the geometry of the underlying problem. However, our method of deriving it as a special case of a general result of \cite{KaufmanOpt} establishes the connection between these studies. 
\end{remark} 
%\begin{proof}{}
%Recall the definition from Lemma \ref{Kaufmann}, 
%\beqn
%T^*(\theta)^{-1} = \sup\limits_{\underline{w}\in \mathcal{P}_K}\inf\limits_{\xi\in Alt(\theta)}\sum\limits_{a=1}^{K}w_ad(\mathcal{N}(\theta^Tx_a,1/2),\mathcal{N}(\xi^Tx_a,1/2)),
%\eeqn
%where $d(.,.)$ is the KL divergence between any two distributions. Hence, we have,
%\begin{align*}
%T^*(\theta)^{-1} =& \sup\limits_{\underline{w}\in \mathcal{P}_K}\inf\limits_{\xi\in Alt(\theta)}\sum\limits_{a=1}^{K}w_a(\theta^Tx_a - \xi^Tx_a)^2\\
%=&  \sup\limits_{\underline{w}\in \mathcal{P}_K}\min\limits_{a'\neq 1}\inf\limits_{\xi: \xi^Tx_a' \geq \xi^Tx_1+\epsilon}\sum\limits_{a=1}^{K}w_a(\theta^Tx_a - \xi^Tx_a)^2
%\end{align*}
%for some $\epsilon >0.$  We will first consider the inner part of the expression above (a convex program), which can be re-written as 
%\beq
%\inf\limits_{\xi: \xi^Tx_a' \geq \xi^Tx_1+\epsilon}(\theta-\xi)^TW(\theta-\xi)
%\eeq
%where $W$ is defined as in the theorem. Writing the Lagrangian, we get
%\beqn
%\mathcal{L}(\xi, \lambda) = (\theta-\xi)^TW(\theta-\xi) -\lambda(\xi^Tx_a' - \xi^Tx_1-\epsilon).
%\eeqn
%Setting $\Delta_{\xi}\mathcal{L}(\xi, \lambda)=0$, we get
%\begin{align*}
%\Delta_{\xi}\mathcal{L}(\xi, \lambda):& -2W\theta + 2W\xi -\lambda(x_{a'}-x_1)= 0\\
%\Rightarrow \xi &= \theta +\frac{\lambda}{2}W^{-1}(x_{a'}-x_1).
%\end{align*}
%Substituting this value of $\xi$ into the Lagrangian, we obtain:
%\begin{flalign*}
%\begin{split}
% \mathcal{L}(\lambda)&= \theta^TW\theta -2\theta^TW(\theta +\frac{\lambda}{2}W^{-1}(x_{a'}-x_1)) \\& +(\theta +\frac{\lambda}{2}W^{-1}(x_{a'}-x_1))^TW(\theta +\frac{\lambda}{2}W^{-1}(x_{a'}-x_1)) \\& -\lambda((\theta +\frac{\lambda}{2}W^{-1}(x_{a'}-x_1))^T(x_{a'}-x_1)-\epsilon)\\
%\end{split}\\
%&=-\frac{\lambda^2}{4} (x_{a'}-x_1)^TW^{-1}(x_{a'}-x_1) -\lambda(\theta^T(x_{a'}-x_1)) + \lambda \epsilon.
%\end{flalign*}
%Setting $\Delta_{\lambda}\mathcal{L}(\lambda) =0,$
%\beq
%\frac{\lambda}{2} = \frac{\epsilon +\Delta_{a'}}{\norm{(x_{a'}-x_1)}_{W^{-1}}^2}.
%\eeq
%Hence, we get :
%\beq
%\xi^* = \theta + \frac{\epsilon +\Delta_{a'}}{\norm{(x_{a'}-x_1)}_{W^{-1}}^2}W^{-1}(x_{a'}-x_1).
%\eeq
%Using this value of $\xi$ in the objective we get,
%\begin{align*}
%T^*(\theta)^{-1} &= \sup\limits_{\underline{w}\in \mathcal{P}_K}\min\limits_{a'\neq 1} \frac{(\epsilon +\Delta_{a'})^2}{\norm{(x_{a'}-x_1)}_{W^{-1}}^2}\\
%& \leq \sup\limits_{\underline{w}\in \mathcal{P}_K} \frac{(\Delta_{min}+\epsilon)^2}{\norm{(x_{a'}-x_1)}_{W^{-1}}^2}\\
%&= \frac{(\Delta_{min}+\epsilon)^2}{\inf\limits_{\underline{w}\in \mathcal{P}_K}\norm{x_2-x_1}_{W^{-1}}^2}.
%\end{align*}
%Putting this into Lemma \ref{Kaufmann},  and taking $\epsilon \to 0$, completes the proof.
%\end{proof}

\subsection{Interpretation of $H_G$}
For interpreting $H_G$, we introduce the notion of an oracle, which knows the actual home cone of $\theta^*$ (or equivalently, the index of the best arm). For any \textit{fixed} strategy $w\in \mathcal{P}_K$ (i.e., a strategy which pulls arms according to the fixed distribution $w, \forall t\geq 0$), and for any suboptimal arm $a$, the term $\frac{\norm{x_a-x_{a^*}}^2_{W^{-1}}}{\Delta_{a}^2}$ represents the time taken by that static strategy to recognize the suboptimality of arm $a$. The oracle's strategy is a fixed strategy $w^*$ which minimizes the time taken to eliminate the last suboptimal arm, i.e., the arm which takes the longest to get eliminated under the strategy $w^*$.

We interpret  $H_G$ with the well-known case of stochastic multi-armed bandits with independent arms. We first note that in this case, $d=K,  \theta=(\mu_1,\mu_2,\ldots,\mu_K)$ and $\mathcal{X}\equiv\{e_1,e_2,\ldots,e_K \}$ which are the standard unit vectors.  We have the following result:
\begin{lemma}\label{lemma:interpretation of T}
\beq
\sum\limits_{a=1}^{K} \frac{1}{\Delta_a^2} \leq H_G^{\theta} \leq 2\sum\limits_{a=1}^{K} \frac{1}{\Delta_a^2},
\eeq
\end{lemma}
where we put $\theta$ as a superscript of $H_G$ to emphasize that it is a function of the unknown parameter $\theta$. 
Proof of this lemma is included in the Appendix \ref{proof of interpretation of T}.
 \par We aim to design an algorithm which competes with an oracle which, for a given problem,  plays $w^*, \forall t$ and achieves the sample complexity lower bound of $H_G$. In fact, we will show that the proposed algorithm \ref{alg:Main} achieves $H_G$ in the cases that we analyze.

% % % % % % % % % % % % % % % % % % % % % % % % % %
